Fusion Subspace Clustering for Incomplete Data

This paper introduces {\em fusion subspace clustering}, a novel method to learn low-dimensional structures that approximate large scale yet highly incomplete data. The main idea is to assign each datum to a subspace of its own, and minimize the distance between the subspaces of all data, so that subspaces of the same cluster get {\em fused} together. Our method allows low, high, and even full-rank data; it directly accounts for noise, and its sample complexity approaches the information-theoretic limit. In addition, our approach provides a natural model selection {\em clusterpath}, and a direct completion method. We give convergence guarantees, analyze computational complexity, and show through extensive experiments on real and synthetic data that our approach performs comparably to the state-of-the-art with complete data, and dramatically better if data is missing.

==> Figures/FiguresOther/Clusterpath.tex <==
% Created by tikzDevice version 0.12.3 on 2020-05-25 17:57:32
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (180.67,144.54);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (180.68,144.54);
\end{scope}
\begin{scope}
\path[clip] ( 25.09, 28.18) rectangle (175.17,125.77);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 25.09, 28.18) rectangle (175.17,125.77);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 25.09, 45.55) --
	(175.17, 45.55);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 25.09, 71.41) --
	(175.17, 71.41);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 25.09, 97.28) --
	(175.17, 97.28);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 25.09,123.14) --
	(175.17,123.14);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 48.32, 28.18) --
	( 48.32,125.77);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 81.13, 28.18) --
	( 81.13,125.77);

\path[draw=drawColor,line width= 0.3pt,line join=round] (115.68, 28.18) --
	(115.68,125.77);

\path[draw=drawColor,line width= 0.3pt,line join=round] (150.22, 28.18) --
	(150.22,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.09, 32.62) --
	(175.17, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.09, 58.48) --
	(175.17, 58.48);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.09, 84.35) --
	(175.17, 84.35);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.09,110.21) --
	(175.17,110.21);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.78, 28.18) --
	( 32.78,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.86, 28.18) --
	( 63.86,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.41, 28.18) --
	( 98.41,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] (132.95, 28.18) --
	(132.95,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.49, 28.18) --
	(167.49,125.77);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 31.91, 32.62) rectangle ( 33.64, 89.26);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 35.37, 32.62) rectangle ( 37.09, 71.15);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.82, 32.62) rectangle ( 40.55, 54.86);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 42.27, 32.62) rectangle ( 44.00, 82.28);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 45.73, 32.62) rectangle ( 47.46,100.90);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 49.18, 32.62) rectangle ( 50.91,102.97);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 52.64, 32.62) rectangle ( 54.36,116.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 56.09, 32.62) rectangle ( 57.82,121.33);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 59.55, 32.62) rectangle ( 61.27,113.83);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 63.00, 32.62) rectangle ( 64.73,105.30);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 66.45, 32.62) rectangle ( 68.18,101.42);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 69.91, 32.62) rectangle ( 71.64, 86.41);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 73.36, 32.62) rectangle ( 75.09, 78.14);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 76.82, 32.62) rectangle ( 78.54, 69.09);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 80.27, 32.62) rectangle ( 82.00, 59.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 83.72, 32.62) rectangle ( 85.45, 56.15);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 87.18, 32.62) rectangle ( 88.91, 51.50);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 90.63, 32.62) rectangle ( 92.36, 49.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 94.09, 32.62) rectangle ( 95.81, 47.88);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 97.54, 32.62) rectangle ( 99.27, 42.19);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (101.00, 32.62) rectangle (102.72, 40.12);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (104.45, 32.62) rectangle (106.18, 41.93);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (107.90, 32.62) rectangle (109.63, 37.27);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (111.36, 32.62) rectangle (113.09, 37.53);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (114.81, 32.62) rectangle (116.54, 36.50);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (118.27, 32.62) rectangle (119.99, 35.72);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (121.72, 32.62) rectangle (123.45, 34.43);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (125.18, 32.62) rectangle (126.90, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (128.63, 32.62) rectangle (130.36, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (132.08, 32.62) rectangle (133.81, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (135.54, 32.62) rectangle (137.27, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (138.99, 32.62) rectangle (140.72, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (142.45, 32.62) rectangle (144.17, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (145.90, 32.62) rectangle (147.63, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (149.35, 32.62) rectangle (151.08, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (152.81, 32.62) rectangle (154.54, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (156.26, 32.62) rectangle (157.99, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (159.72, 32.62) rectangle (161.44, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (163.17, 32.62) rectangle (164.90, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (166.63, 32.62) rectangle (168.35, 32.87);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 31.91, 32.62) rectangle ( 33.64, 57.45);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 35.37, 32.62) rectangle ( 37.09, 54.60);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.82, 32.62) rectangle ( 40.55, 50.46);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 42.27, 32.62) rectangle ( 44.00, 48.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 45.73, 32.62) rectangle ( 47.46, 43.74);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 49.18, 32.62) rectangle ( 50.91, 46.58);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 52.64, 32.62) rectangle ( 54.36, 42.19);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 56.09, 32.62) rectangle ( 57.82, 40.12);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 59.55, 32.62) rectangle ( 61.27, 38.05);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 63.00, 32.62) rectangle ( 64.73, 39.08);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 66.45, 32.62) rectangle ( 68.18, 38.05);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 69.91, 32.62) rectangle ( 71.64, 36.75);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 73.36, 32.62) rectangle ( 75.09, 37.01);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 76.82, 32.62) rectangle ( 78.54, 36.24);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 80.27, 32.62) rectangle ( 82.00, 35.46);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 83.72, 32.62) rectangle ( 85.45, 34.68);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 87.18, 32.62) rectangle ( 88.91, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 90.63, 32.62) rectangle ( 92.36, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 94.09, 32.62) rectangle ( 95.81, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 97.54, 32.62) rectangle ( 99.27, 35.20);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (101.00, 32.62) rectangle (102.72, 34.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (104.45, 32.62) rectangle (106.18, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (107.90, 32.62) rectangle (109.63, 34.43);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (111.36, 32.62) rectangle (113.09, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (114.81, 32.62) rectangle (116.54, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (118.27, 32.62) rectangle (119.99, 34.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (121.72, 32.62) rectangle (123.45, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (125.18, 32.62) rectangle (126.90, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (128.63, 32.62) rectangle (130.36, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (132.08, 32.62) rectangle (133.81, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (135.54, 32.62) rectangle (137.27, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (138.99, 32.62) rectangle (140.72, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (142.45, 32.62) rectangle (144.17, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (145.90, 32.62) rectangle (147.63, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (149.35, 32.62) rectangle (151.08, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (152.81, 32.62) rectangle (154.54, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (156.26, 32.62) rectangle (157.99, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (159.72, 32.62) rectangle (161.44, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (163.17, 32.62) rectangle (164.90, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (166.63, 32.62) rectangle (168.35, 33.13);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 18.23, 29.98) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 18.23, 55.84) {1};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 18.23, 81.71) {2};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 18.23,107.57) {3};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 22.34, 32.62) --
	( 25.09, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 22.34, 58.48) --
	( 25.09, 58.48);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 22.34, 84.35) --
	( 25.09, 84.35);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 22.34,110.21) --
	( 25.09,110.21);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 32.78, 25.43) --
	( 32.78, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 63.86, 25.43) --
	( 63.86, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 98.41, 25.43) --
	( 98.41, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] (132.95, 25.43) --
	(132.95, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.49, 25.43) --
	(167.49, 28.18);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 32.78, 17.07) {$\mathbb{U}_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 63.86, 17.07) {$\mathbb{U}_8$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 98.41, 17.07) {$\mathbb{U}_{16}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at (132.95, 17.07) {$\mathbb{U}_{24}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at (167.49, 17.07) {$\mathbb{U}_{32}$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at (100.13,  7.27) {Subspaces};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at ( 11.79, 76.97) {$\log \lambda$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 91.32, 68.93) rectangle (168.98,124.05);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 96.82, 88.88) rectangle (111.28,103.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.24, 90.31) rectangle (109.85,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.24, 90.31) rectangle (109.85,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 96.82, 74.43) rectangle (111.28, 88.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.24, 75.85) rectangle (109.85, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.24, 75.85) rectangle (109.85, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at (116.78, 93.46) {Outer-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at (116.78, 79.01) {Intra-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (100.13,132.98) {Clusterpath};
\end{scope}
\end{tikzpicture}


==> Figures/FiguresOther/DistanceMatrix.tex <==
% Created by tikzDevice version 0.12.3 on 2020-05-25 15:55:37
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (144.54,144.54);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (144.54,144.54);
\end{scope}
\begin{scope}
\path[clip] ( 33.28, 28.18) rectangle (139.04,125.77);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 33.28, 28.18) rectangle (139.04,125.77);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 33.28, 55.25) --
	(139.04, 55.25);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 33.28,100.51) --
	(139.04,100.51);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 61.82, 28.18) --
	( 61.82,125.77);

\path[draw=drawColor,line width= 0.3pt,line join=round] (109.28, 28.18) --
	(109.28,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 33.28, 32.62) --
	(139.04, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 33.28, 77.88) --
	(139.04, 77.88);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 33.28,123.14) --
	(139.04,123.14);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 38.69, 28.18) --
	( 38.69,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.94, 28.18) --
	( 84.94,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] (133.62, 28.18) --
	(133.62,125.77);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.09, 32.62) rectangle ( 39.30, 89.26);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 40.52, 32.62) rectangle ( 41.74, 71.15);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 42.95, 32.62) rectangle ( 44.17, 54.86);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 45.39, 32.62) rectangle ( 46.61, 82.28);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 47.82, 32.62) rectangle ( 49.04,100.90);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 50.26, 32.62) rectangle ( 51.47,102.97);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 52.69, 32.62) rectangle ( 53.91,116.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 55.12, 32.62) rectangle ( 56.34,121.33);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 57.56, 32.62) rectangle ( 58.78,113.83);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 59.99, 32.62) rectangle ( 61.21,105.30);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 62.43, 32.62) rectangle ( 63.64,101.42);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 64.86, 32.62) rectangle ( 66.08, 86.41);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 67.29, 32.62) rectangle ( 68.51, 78.14);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 69.73, 32.62) rectangle ( 70.95, 69.09);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 72.16, 32.62) rectangle ( 73.38, 59.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 74.60, 32.62) rectangle ( 75.81, 56.15);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 77.03, 32.62) rectangle ( 78.25, 51.50);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 79.47, 32.62) rectangle ( 80.68, 49.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 81.90, 32.62) rectangle ( 83.12, 47.88);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 84.33, 32.62) rectangle ( 85.55, 42.19);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 86.77, 32.62) rectangle ( 87.98, 40.12);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 89.20, 32.62) rectangle ( 90.42, 41.93);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 91.64, 32.62) rectangle ( 92.85, 37.27);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 94.07, 32.62) rectangle ( 95.29, 37.53);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 96.50, 32.62) rectangle ( 97.72, 36.50);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.94, 32.62) rectangle (100.16, 35.72);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (101.37, 32.62) rectangle (102.59, 34.43);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (103.81, 32.62) rectangle (105.02, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (106.24, 32.62) rectangle (107.46, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (108.67, 32.62) rectangle (109.89, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (111.11, 32.62) rectangle (112.33, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (113.54, 32.62) rectangle (114.76, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (115.98, 32.62) rectangle (117.19, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (118.41, 32.62) rectangle (119.63, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (120.85, 32.62) rectangle (122.06, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (123.28, 32.62) rectangle (124.50, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (125.71, 32.62) rectangle (126.93, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (128.15, 32.62) rectangle (129.36, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (130.58, 32.62) rectangle (131.80, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (133.02, 32.62) rectangle (134.23, 32.87);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.09, 32.62) rectangle ( 39.30, 57.45);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 40.52, 32.62) rectangle ( 41.74, 54.60);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 42.95, 32.62) rectangle ( 44.17, 50.46);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 45.39, 32.62) rectangle ( 46.61, 48.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 47.82, 32.62) rectangle ( 49.04, 43.74);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 50.26, 32.62) rectangle ( 51.47, 46.58);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 52.69, 32.62) rectangle ( 53.91, 42.19);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 55.12, 32.62) rectangle ( 56.34, 40.12);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 57.56, 32.62) rectangle ( 58.78, 38.05);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 59.99, 32.62) rectangle ( 61.21, 39.08);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 62.43, 32.62) rectangle ( 63.64, 38.05);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 64.86, 32.62) rectangle ( 66.08, 36.75);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 67.29, 32.62) rectangle ( 68.51, 37.01);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 69.73, 32.62) rectangle ( 70.95, 36.24);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 72.16, 32.62) rectangle ( 73.38, 35.46);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 74.60, 32.62) rectangle ( 75.81, 34.68);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 77.03, 32.62) rectangle ( 78.25, 34.94);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 79.47, 32.62) rectangle ( 80.68, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 81.90, 32.62) rectangle ( 83.12, 32.87);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 84.33, 32.62) rectangle ( 85.55, 35.20);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 86.77, 32.62) rectangle ( 87.98, 34.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 89.20, 32.62) rectangle ( 90.42, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 91.64, 32.62) rectangle ( 92.85, 34.43);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 94.07, 32.62) rectangle ( 95.29, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 96.50, 32.62) rectangle ( 97.72, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 98.94, 32.62) rectangle (100.16, 34.17);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (101.37, 32.62) rectangle (102.59, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (103.81, 32.62) rectangle (105.02, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (106.24, 32.62) rectangle (107.46, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (108.67, 32.62) rectangle (109.89, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (111.11, 32.62) rectangle (112.33, 33.39);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (113.54, 32.62) rectangle (114.76, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (115.98, 32.62) rectangle (117.19, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (118.41, 32.62) rectangle (119.63, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (120.85, 32.62) rectangle (122.06, 33.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (123.28, 32.62) rectangle (124.50, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (125.71, 32.62) rectangle (126.93, 33.65);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (128.15, 32.62) rectangle (129.36, 33.13);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (130.58, 32.62) rectangle (131.80, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (133.02, 32.62) rectangle (134.23, 33.13);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.32, 29.98) {$\mathbb{U}_{96}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.32, 75.24) {$\mathbb{U}_{48}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.32,120.51) {$\mathbb{U}_1$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 30.53, 32.62) --
	( 33.28, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 30.53, 77.88) --
	( 33.28, 77.88);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 30.53,123.14) --
	( 33.28,123.14);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 38.69, 25.43) --
	( 38.69, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 84.94, 25.43) --
	( 84.94, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] (133.62, 25.43) --
	(133.62, 28.18);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 38.69, 17.07) {$\mathbb{U}_1$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 84.94, 17.07) {$\mathbb{U}_{48}$};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at (133.62, 17.07) {$\mathbb{U}_{96}$};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at ( 86.16,  7.27) {Subspaces};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at ( 11.79, 76.97) {Subspaces};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);

\path[] ( 68.48, 68.93) rectangle (146.14,124.05);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);

\path[] ( 73.98, 88.88) rectangle ( 88.44,103.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.41, 90.31) rectangle ( 87.01,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.41, 90.31) rectangle ( 87.01,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);

\path[] ( 73.98, 74.43) rectangle ( 88.44, 88.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.41, 75.85) rectangle ( 87.01, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.41, 75.85) rectangle ( 87.01, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 93.94, 93.46) {Outer-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 93.94, 79.01) {Intra-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (144.54,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at ( 86.16,132.98) {Yale ($\gamma=1$)};
\end{scope}
\end{tikzpicture}


==> Figures/FiguresOther/YaleOuterIntra.tex <==
% Created by tikzDevice version 0.12.3 on 2020-05-25 18:02:35
% !TEX encoding = UTF-8 Unicode
\begin{tikzpicture}[x=1pt,y=1pt]
\definecolor{fillColor}{RGB}{255,255,255}
\path[use as bounding box,fill=fillColor,fill opacity=0.00] (0,0) rectangle (180.67,144.54);
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{255,255,255}
\definecolor{fillColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.6pt,line join=round,line cap=round,fill=fillColor] (  0.00,  0.00) rectangle (180.68,144.54);
\end{scope}
\begin{scope}
\path[clip] ( 28.02, 28.18) rectangle (175.17,125.77);
\definecolor{fillColor}{gray}{0.92}

\path[fill=fillColor] ( 28.02, 28.18) rectangle (175.17,125.77);
\definecolor{drawColor}{RGB}{255,255,255}

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 28.02, 41.97) --
	(175.17, 41.97);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 28.02, 60.69) --
	(175.17, 60.69);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 28.02, 79.41) --
	(175.17, 79.41);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 28.02, 98.12) --
	(175.17, 98.12);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 28.02,116.84) --
	(175.17,116.84);

\path[draw=drawColor,line width= 0.3pt,line join=round] ( 67.73, 28.18) --
	( 67.73,125.77);

\path[draw=drawColor,line width= 0.3pt,line join=round] (133.77, 28.18) --
	(133.77,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.02, 32.62) --
	(175.17, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.02, 51.33) --
	(175.17, 51.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.02, 70.05) --
	(175.17, 70.05);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.02, 88.77) --
	(175.17, 88.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 28.02,107.48) --
	(175.17,107.48);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 35.56, 28.18) --
	( 35.56,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 99.91, 28.18) --
	( 99.91,125.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.64, 28.18) --
	(167.64,125.77);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 34.71, 32.62) rectangle ( 36.41, 33.89);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.10, 32.62) rectangle ( 39.79, 82.55);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 41.49, 32.62) rectangle ( 43.18,121.33);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 44.87, 32.62) rectangle ( 46.57,110.85);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 48.26, 32.62) rectangle ( 49.95, 70.80);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 51.65, 32.62) rectangle ( 53.34, 50.21);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 55.03, 32.62) rectangle ( 56.73, 40.40);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 58.42, 32.62) rectangle ( 60.11, 36.06);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 61.81, 32.62) rectangle ( 63.50, 33.89);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 65.19, 32.62) rectangle ( 66.89, 33.29);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 68.58, 32.62) rectangle ( 70.27, 32.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 71.97, 32.62) rectangle ( 73.66, 32.69);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.35, 32.62) rectangle ( 77.05, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 78.74, 32.62) rectangle ( 80.43, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 82.13, 32.62) rectangle ( 83.82, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 85.51, 32.62) rectangle ( 87.21, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 88.90, 32.62) rectangle ( 90.59, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 92.29, 32.62) rectangle ( 93.98, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 95.67, 32.62) rectangle ( 97.37, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.06, 32.62) rectangle (100.75, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (102.45, 32.62) rectangle (104.14, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (105.83, 32.62) rectangle (107.53, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (109.22, 32.62) rectangle (110.91, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (112.61, 32.62) rectangle (114.30, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (115.99, 32.62) rectangle (117.69, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (119.38, 32.62) rectangle (121.07, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (122.77, 32.62) rectangle (124.46, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (126.15, 32.62) rectangle (127.85, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (129.54, 32.62) rectangle (131.23, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (132.93, 32.62) rectangle (134.62, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (136.31, 32.62) rectangle (138.01, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (139.70, 32.62) rectangle (141.39, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (143.09, 32.62) rectangle (144.78, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (146.47, 32.62) rectangle (148.17, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (149.86, 32.62) rectangle (151.55, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (153.25, 32.62) rectangle (154.94, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (156.63, 32.62) rectangle (158.33, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (160.02, 32.62) rectangle (161.71, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (163.41, 32.62) rectangle (165.10, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (166.79, 32.62) rectangle (168.49, 32.62);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 34.71, 32.62) rectangle ( 36.41, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 38.10, 32.62) rectangle ( 39.79, 39.88);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 41.49, 32.62) rectangle ( 43.18, 39.28);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 44.87, 32.62) rectangle ( 46.57, 38.38);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 48.26, 32.62) rectangle ( 49.95, 37.33);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 51.65, 32.62) rectangle ( 53.34, 35.76);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 55.03, 32.62) rectangle ( 56.73, 36.81);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 58.42, 32.62) rectangle ( 60.11, 34.79);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 61.81, 32.62) rectangle ( 63.50, 35.01);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 65.19, 32.62) rectangle ( 66.89, 34.34);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 68.58, 32.62) rectangle ( 70.27, 34.64);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 71.97, 32.62) rectangle ( 73.66, 33.89);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 75.35, 32.62) rectangle ( 77.05, 33.74);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 78.74, 32.62) rectangle ( 80.43, 34.19);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 82.13, 32.62) rectangle ( 83.82, 33.36);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 85.51, 32.62) rectangle ( 87.21, 33.21);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 88.90, 32.62) rectangle ( 90.59, 33.36);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 92.29, 32.62) rectangle ( 93.98, 33.06);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 95.67, 32.62) rectangle ( 97.37, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.06, 32.62) rectangle (100.75, 33.51);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (102.45, 32.62) rectangle (104.14, 32.99);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (105.83, 32.62) rectangle (107.53, 32.99);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (109.22, 32.62) rectangle (110.91, 32.99);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (112.61, 32.62) rectangle (114.30, 32.84);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (115.99, 32.62) rectangle (117.69, 32.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (119.38, 32.62) rectangle (121.07, 33.21);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (122.77, 32.62) rectangle (124.46, 32.99);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (126.15, 32.62) rectangle (127.85, 32.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (129.54, 32.62) rectangle (131.23, 33.06);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (132.93, 32.62) rectangle (134.62, 32.69);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (136.31, 32.62) rectangle (138.01, 32.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (139.70, 32.62) rectangle (141.39, 32.84);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (143.09, 32.62) rectangle (144.78, 32.84);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (146.47, 32.62) rectangle (148.17, 32.84);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (149.86, 32.62) rectangle (151.55, 32.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (153.25, 32.62) rectangle (154.94, 32.91);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (156.63, 32.62) rectangle (158.33, 32.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (160.02, 32.62) rectangle (161.71, 32.62);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (163.41, 32.62) rectangle (165.10, 32.77);

\path[draw=drawColor,line width= 1.1pt,line cap=rect] (166.79, 32.62) rectangle (168.49, 32.62);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.33, 32.62) {0};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.33, 51.33) {500};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.33, 70.05) {1000};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.33, 88.77) {1500};

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.77] at ( 22.33,107.48) {2000};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.27, 32.62) --
	( 28.02, 32.62);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.27, 51.33) --
	( 28.02, 51.33);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.27, 70.05) --
	( 28.02, 70.05);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.27, 88.77) --
	( 28.02, 88.77);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 25.27,107.48) --
	( 28.02,107.48);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{gray}{0.20}

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 35.56, 25.43) --
	( 35.56, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] ( 99.91, 25.43) --
	( 99.91, 28.18);

\path[draw=drawColor,line width= 0.6pt,line join=round] (167.64, 25.43) --
	(167.64, 28.18);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{190,190,190}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 35.56, 17.07) {0};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at ( 99.91, 17.07) {.01};

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.78] at (167.64, 17.07) {.02};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at (101.60,  7.27) {Gaussian Kernel};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,rotate= 90.00,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.91] at ( 11.79, 76.97) {Counts};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 92.20, 68.93) rectangle (169.86,124.05);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 97.70, 88.88) rectangle (112.16,103.34);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.12, 90.31) rectangle (110.73,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,255}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.12, 90.31) rectangle (110.73,101.92);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);

\path[] ( 97.70, 74.43) rectangle (112.16, 88.88);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.12, 75.85) rectangle (110.73, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\path[draw=drawColor,line width= 1.1pt,line cap=rect] ( 99.12, 75.85) rectangle (110.73, 87.46);
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at (117.66, 93.46) {Outer-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base west,inner sep=0pt, outer sep=0pt, scale=  0.77] at (117.66, 79.01) {Intra-Cluster};
\end{scope}
\begin{scope}
\path[clip] (  0.00,  0.00) rectangle (180.67,144.54);
\definecolor{drawColor}{RGB}{0,0,0}

\node[text=drawColor,anchor=base,inner sep=0pt, outer sep=0pt, scale=  0.88] at (101.60,132.98) {Yale Dataset};
\end{scope}
\end{tikzpicture}

